Filtered Direct Preference Optimization

Reinforcement learning from human feedback (RLHF) plays a crucial role in aligning language models with human preferences. While the significance of dataset quality is generally recognized, explicit investigations into its impact within the RLHF framework, to our knowledge, have been limited. This paper addresses the issue of text quality within the preference dataset by focusing on direct preference optimization (DPO), an increasingly adopted reward-model-free RLHF method. We confirm that text quality significantly influences the performance of models optimized with DPO more than those optimized with reward-model-based RLHF. Building on this new insight, we propose an extension of DPO, termed filtered direct preference optimization (fDPO). fDPO uses a trained reward model to monitor the quality of texts within the preference dataset during DPO training. Samples of lower quality are discarded based on comparisons with texts generated by the model being optimized, resulting in a more accurate dataset. Experimental results demonstrate that fDPO enhances the final model performance. Our code is available at https://github.com/CyberAgentAILab/filtered-dpo.

==> sec_experiment_old.tex <==
\section{Experiments}
\label{sec:experiment}
%%%
We first detail our experimental setup, including the pretrained models in Section~\ref{sec:exp_model} and the data in Section~\ref{sec:exp_data}.
%
We then evaluate the impact of data quality on DPO in Section~\ref{sec:exp_preliminary} and the effectiveness of fDPO in Sections \ref{sec:exp_main} and \ref{sec:exp_detailed} in the context of instruction following tasks,
focusing on the ability to generate appropriate responses to prompts. 
%
For our baseline comparison, we include a DPO implementation from the Transformer Reinforcement Learning (TRL) library.\footnote{https://github.com/huggingface/trl}
%
%The instruction following task involves generating appropriate responses to instructions (and inputs) as prompts, serving as a standard test for language model proficiency.
%


%%%
\subsection{Pretrained Models}
\label{sec:exp_model}
In our experiments, we employed pretrained LMs provided in the
Pythia suite by \citet{biderman2023pythia} of two different sizes: 1.4B and 160M models. 
%
In Section \ref{sec:exp_main}, we present the primary findings of our study using a 1.4B-sized LM to highlight the effectiveness of fDPO in an LLM.
%
Due to computational resource constraints, a comprehensive examination of the 160M LM is provided in Section \ref{sec:exp_detailed}.
%
In the preliminary setup, each LM was subjected to SFT using the demonstration dataset from AlpacaFarm \citep{AlpacaFarm23}. 
%
These prepared LMs, denoted as $\pi_\theta$, were then used as the initial LMs for our experiments.
%

%%%
For the (proxy) RM, we used Pythia models of varying sizes: 14M, 70M, and 160M models.
%
To circumvent the high costs associated with human evaluation, similar to other studies \cite{AlpacaFarm23, DPO}, we utilized a large-scale human preference model as the gold RM. Specifically, ``OpenAssistant/reward-model-deberta-v3-large-v2''\footnote{https://huggingface.co/OpenAssistant/reward-model-deberta-v3-large-v2} model was employed for this purpose.
%


%%%
\subsection{Data}
\label{sec:exp_data}
%%%
We utilized the AlpacaFarm instruction dataset \citep{AlpacaFarm23} for our experiments. 
%
The dataset consisted of 20,000 training samples. 
%
For evaluation, a random selection of 200 samples from in a pool of 2000 was used in each independent run to ensure consistency and unbiased results.
%

%%%
The baseline DPO and our proposed fDPO used the same data to ensure a fair comparison.
%
This means that in fDPO, both the RM and the LM were trained using an identical dataset. 
%

%%%
Given our focus on dataset quality, we employed gold RM and BoN sampling \citep{bon20, bon21} to create three types of pairwise preference datasets:
%
\vspace{-1mm}
%%%
\paragraph{Low-quality dataset.}
This dataset was created using the conventional manner. 
%
For each prompt $x$, the LM $\pi_\theta$ generated two responses.
%
These responses were then evaluated by the gold RM, with the higher-scoring response designated as $\chosen$ and the other as $\rejected$. 
%
This formed the preference dataset $\mathcal{D}$ samples $(x, \chosen, \rejected)$. 
%
For brevity, this dataset is referred to as the `low dataset'.
%
\vspace{-1mm}
%%%
\paragraph{High-quality dataset.}
Adopting the approach from \citep{west-of-n24}, we used BoN sampling to create responses of higher quality. 
%
Specifically, for each prompt $x$, the LM $\pi_\theta$ generated $16$ responses.
%
These responses were then evaluated by the gold RM, and the highest-scoring response was selected as $\chosen$, with one randomly selected from the remaining 15 responses labeled as $\rejected$.
%
Due to the probabilistic nature of outputs of $\pi_\theta$, this approach is likely to yield $\chosen$ responses of higher quality (as indicated by gold RM scores) compared to the $\chosen$ responses in the low-quality dataset. 
%
For simplicity, this dataset is referred to as the `high dataset'.
%
\vspace{-1mm}
%%%
\paragraph{Mix-quality dataset.}
This dataset was created by mixing the low-quality and high-quality datasets in a 50/50 ratio, ensuring no overlap in prompts between the two. 
%
This dataset is referred to as the `mix dataset'.

%%%
We provide the evaluation scores of the gold RM for these datasets in Table \ref{tab:eval_pref_dataset} in Appendix \ref{sec:exp_appendix}.


%%%
\subsection{Effect of Data Quality to Performance of RLHF and DPO}
\label{sec:exp_preliminary}
%%%
Our preliminary experiment investigates the sensitivities of (RM-based) RLHF and (RM-free) DPO to the quality of the datasets employed with the 160M-sized LM.
%
Here, we used the high-quality and mixed-quality datasets. 
%
We used an RLHF implementation in the TRL library, in which a 70M-sized RM is trained and then used for RL fine-tuning.
%
The evaluation is based on three independent runs, with each run employing different evaluation prompts that could vary ranges of the average of gold rewards.
%
For a coherent comparison, gold rewards are normalized, setting the initial performance of LM to $0.0$ and post-training performance with RLHF or DPO to $1.0$. 

%%%
Figure \ref{fig:teaser} (A) shows the results, where the mean and standard error of the normalized gold reward with three independent runs are presented.
% 
Notably, while DPO experienced a decline in efficacy when trained on the mixed-quality dataset relative to the high-quality one, RLHF showed an intriguing resilience, sustaining comparable performance levels across both datasets.
%
This differential impact starkly highlights the greater susceptibility of DPO to dataset quality, suggesting that the RM-based approach, including fDPO, may offer more stable performance when the preference dataset quality cannot be consistently assured. 
%
All experiments are conducted using a single NVIDIA A100 accelerator. 
%
Further details of the experimental parameters are provided in Table~\ref{tab:experimental_params} in Appendix~\ref{sec:exp_appendix}.


%%%
\subsection{Evaluation of fDPO}
\label{sec:exp_main}
%%%
We evaluate fDPO and DPO when trained using a 1.4B-sized LM $\pi_\theta$ on the mixed-quality dataset, where fDPO used a 160M-sized RM that was trained with the same dataset.
%
The evaluation is based on three independent runs, where the gold reward was normalized with the performance of DPO with high-quality dataset, as in Section \ref{sec:exp_preliminary}.
%
The epoch number for DPO was set to 5, which avoided overoptimization while ensuring the learning convergence. 
%
In the case of fDPO, we adapted the epoch count to double that of DPO, up to 10 epochs, or ceased learning when the remaining sample size was reduced to less than 1\% of the original due to the filtering process, meaning the maximum filtered rate $\gamma=0.99$.
%

Figure \ref{fig:1.4B-mix} present the results of DPO and fDPO. 
%
The results shows that the performance of DPO trained on the high-quality dataset and fDPO trained on the mixed-quality dataset were on par.
%
It indicates that fDPO has successfully circumvented the performance decline typically observed with DPO, thereby showcasing its potential to improve DPO performance where dataset quality is inconsistent.
%demonstrates that fDPO effectively manages the challenges posed by mixed-quality datasets. 
%
Corresponding learning curves are included in Appendix \ref{sec:exp_appendix}. 
%

\begin{figure}[t]
\centering
%\vspace{-5mm}
\includegraphics[width=0.7\linewidth]{figs/fdpo_bar_1_4b.pdf}
%\vspace{-3mm}
\caption{Performance comparison between DPO and fDPO using a 1.4B-sized LM on the mix-quality dataset.}
\label{fig:1.4B-mix}
\end{figure}



\subsection{Detailed Experiments}
\label{sec:exp_detailed}
We delve into an extensive analysis of fDPO using a 160M LM. 
%
We set the number of epochs to $8$ for DPO to ensure convergence, resulting in a maximum of $16$ epochs for fDPO. 
%
We maintained the maximum filtered rate ($\gamma=0.99$) as unchanged.

%%%
\paragraph{Performance comparison with DPO.}
Figure \ref{fig:teaser} (B) illustrates the performances of LMs trained with DPO and fDPO using the mixed-quality dataset.
%
The results are consistent with those obtained from the larger 1.4B-sized LM, reaffirming the advantage of fDPO with the mixed-quality dataset.
%
Additionally, we conducted an experiment using only a low-quality dataset, which revealed a surprising improvement of 7.42\% (standard error: 1.89\%) despite the presumed uniformity of response quality.
%
This improvement suggests it effectively discriminates subtle quality variations, enhancing overall performance by eliminating less optimal data, even within uniformly labeled datasets.
%

%%%
\paragraph{Analysis of configuration parameters.}
%
\begin{figure*}[t]
\hspace{-5mm}
\begin{tabular}{ccc}
\begin{minipage}{.285\textwidth}
\centering
\includegraphics[width=0.92\linewidth]{figs/fdpo_sens_rm.pdf}
%\vspace{-3mm}  
\caption{RM size}
\label{fig:rm-size}
%
\end{minipage}
\hspace{-3mm}
\begin{minipage}{.365\textwidth}
    \centering
    %\hspace{5mm}
    \includegraphics[width=0.97\linewidth]{figs/fdpo_sens_top.pdf}
%    \vspace{-3mm}  
    \caption{Top p sampling}
    \label{fig:top-p}
\end{minipage}
%
\begin{minipage}{.365\textwidth}
    \centering
    \includegraphics[width=0.97\linewidth]{figs/fdpo_sens_margin.pdf}
  %  \vspace{-3mm}   
    \caption{Margin for filtering}
    \label{fig:mergin}
\end{minipage}
\end{tabular}
%\vspace{-1mm}
\end{figure*}

\begin{figure*}[th]
%\vspace{-4mm}
\begin{tabular}{cc}
% \begin{minipage}{.24\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth]{figs/filtered_dataset_filtered_ratio.pdf}
% \caption{filtered ratio}
% \label{fig:enter-label4}
% \end{minipage}
\begin{minipage}{.99\textwidth}
    %\centering
    \hspace{-4mm}
    % \includegraphics[width=1.04\linewidth]{figs/filtered_dataset_eval_gold.pdf}
    \includegraphics[width=1.01\linewidth]{figs/filtered_dataset_eval_gold_all.pdf}
%    \vspace{-4mm}  
    \caption{Unfiltered ratio, accuracy, precision, and recall throughout epochs in fDPO, comparing the effects of no margin ($\epsilon=0$) with various margin levels ($\epsilon>0$) on the filtering condition.}
    \label{fig:filtered-sample}
\end{minipage}
\end{tabular}
\end{figure*}


We investigated various aspects of fDPO, including the size of RMs, the randomness of LMs, and the criteria for the sampling filtering, with the mix-quality dataset.
%
Figure \ref{fig:rm-size} displays the impact of RM size. 
%
Consistent with findings from \cite{InstructGPT}, smaller RMs relative to the LM size yielded better performance.
%
This contrasts with studies advocating larger RMs for improved performance \citep{RMOveropt, RMEnsemble24}, highlighting an area for further detailed analysis.

%%%
Reducing randomness of LMs was hypothesized to enhance fDPO’s performance by minimizing the variance in quality of the LM-generated responses.
%
However, as Figure \ref{fig:top-p} indicates, reducing randomness did not yield improvements, and in some cases, it led to worse performance.
%
This outcome may be attributed to a discrepancy between inference-time and training-time randomness.

%%%
Finally, we explored different criteria for discarding data. 
%
As stated in line 8 of Algorithm 1, the original criterion was discarding a sample even if the reward of the LM-generated response $y$ is only marginally higher than that of $\chosen$ in the dataset. 
%
Considering potential errors in proxy rewards and the probabilistic nature of LMs, we introduced a margin $\epsilon$ to the discarding criterion: $r(x, y) > r(x, \chosen) + \epsilon$. 
%
Figure \ref{fig:mergin} presents the results, showing that a certain margin size can indeed be effective in enhancing fDPO’s performance.






\paragraph{Analysis of filtered samples.}
%%%
We examined how data was selectively discarded throughout the learning process of fDPO with the mix-quality dataset.
%
Figure \ref{fig:filtered-sample} presents the unfiltered ratio, accuracy, precision, and recall at each epoch.
%
The unfiltered ratio reflects the proportion of data that remains after filtering.
%
Accuracy reflects the overall correctness of the filtering decisions, both for deletion and retention of samples, based on their gold reward quality.
%
Precision measures how accurately the samples decided for deletion were actually of lower quality, while recall evaluates the success in identifying and discarding all samples that warranted removal.
%
%
The result of the unfiltered ratio indicates an exponential decay in the number of samples used in each epoch.
%
The consistency of accuracy and precision across epochs suggests that data was discarded with a constant efficiency.
%
The lower precision compared to accuracy can be attributed to the relatively small number of samples that warranted removal.
%
Conversely, recall decreases with progressing epochs. This decline can be tied to the static errors within the proxy RM, leading to consistently overestimated $\chosen$ samples, thus increasing their relative proportion over time.
%
%
The figure contrasts various margin settings with the no-margin condition ($\epsilon=0$), revealing that larger margins lead to slower filtering speeds. Notably, as the margin increases, precision improves at the expense of recall. This trade-off underscores the importance of carefully tuning the margin parameter $\epsilon$ to balance filtering efficacy.















\if0
\subsection{Further Evaluation}



\begin{figure}[t]
\begin{tabular}{cc}
\begin{minipage}{.49\textwidth}
\centering
\includegraphics[width=0.4\linewidth]{figs/fdpo_bar_bo2.pdf}
\caption{normal}
\label{fig:enter-label4}
\end{minipage}
\begin{minipage}{.49\textwidth}

    \centering
    \includegraphics[width=0.9\linewidth]{figs/fdpo_bar_1_4b.pdf}
    \caption{1.4b}
    \label{fig:enter-label5}
\end{minipage}
\end{tabular}
\end{figure}

\fi

